On phase-space integrals with Heaviside functions

We discuss peculiarities that arise in the computation of real-emission contributions to observables that contain Heaviside functions. A prominent example of such a case is the zero-jettiness soft function in SCET, whose calculation at next-to-next-to-next-to-leading order in perturbative QCD is an interesting problem. Since the zero-jettiness soft function distinguishes between emissions into different hemispheres, its definition involves $\theta$-functions of light-cone components of emitted soft partons. This prevents a direct use of multi-loop methods, based on reverse unitarity, for computing the zero-jettiness soft function in high orders of perturbation theory. We propose a way to bypass this problem and illustrate its effectiveness by computing various non-trivial contrbutions to the zero-jettiness soft function at NNLO and N3LO in perturbative QCD.

==> sections/02_definitions.tex <==
\section{Real-emission contributions to the zero-jettiness soft function}
\label{sec:defs}

The zero-jettiness soft function
describes  effects of soft real and virtual partons (quarks and gluons) on the differential
cross section $pp \to V$, where $V$ is a color-singlet final state. 
The softness is enforced by the use of eikonal propagators and vertices in the calculation
of  amplitudes and by removing 
soft-gluon momenta from the energy-momentum conserving $\delta$-function.

We write the bare soft function as a power series in the bare strong coupling constant
\begin{align}
S(\tau) = \sum_{m} \left[\alpha_s\right]^m S^{(m)}(\tau) \,,
\label{eqn:pert_exp_softF}
\end{align}
where
\begin{align}
\left[\alpha_s\right] = \frac{g_{s,b}^2}{16\pi^2} \frac{(4\pi)^{\ep}}{\Gamma(1-\ep)} = \frac{g_{s,b}^2 \Omega^{(d-2)}}{4(2\pi)^{d-1}} = g_{s,b}^2 N_\ep  \,.
\end{align}
At each order in perturbation theory, coefficients $S^{(m)}(\tau)$ receive real-emission and real-virtual contributions.\footnote{Purely virtual contributions vanish in dimensional regularization.} As we will discuss in what follows, integration over momenta of real
gluons is complicated as  the definition of the soft function
involves $\theta$-functions of light-cone coordinates of the emitted
partons.   The goal of this paper is to discuss how such integrals can be computed.  In particular,
we discuss an extension of  IBP methods to such integrals. 


For the sake of definiteness, we consider gluon real-emission contributions only. 
That is, at $m$-th order in the expansion in $\alpha_s$,
we consider the partonic process $a \bar{a} \to V + m g$, where $a\bar{a} \in \{ gg, q \bar{q} \}$.
We write
\be
S^{(m)}(\tau) = S^{(mg)}(\tau) + ... 
\ee
where ellipses stand for real-virtual contributions\footnote{And, e.g.~quark emission contributions.} and 
\be
S^{(mg)}(\tau) = \frac{(N_\ep)^{-m}}{m!} 
\int \left( \prod_{j=1}^{m}  [{\rm d} k_j ] \right)
\delta ( \tau - {\cal T} ) \; {\rm Eik}_{mg}(k_1,\dots,k_m,n,\bar n).
\label{eq2.1}
\ee
In  Eq.~(\ref{eq2.1})
 $1/m!$ is the normalization  factor, ${\cal T}$ is the jettiness variable defined as 
\be
   {\cal T} = \sum \limits_{j=1}^{m} {\rm min}_{q \in \{ n,\bar n \}} \left [ \frac{2 (q k_j)}{(n \bar n)}  \right ],
   \label{eq2.2}
\ee
and ``${\rm Eik}_{mg}$'' is the eikonal function that describes  emission of $m$ soft real gluons.
The  phase-space elements read
\begin{align}
[\DIFFL k_i] = \frac{\DIFFD \VEC{k}_i}{(2\pi)^{d-1}2k_i^0}.
\end{align}
We use the Sudakov parametrization  of the gluons' momenta and write 
\be
k_i= \frac{\alpha_i}{2} n + \frac{\beta_i}{2} \bar n + k_{\perp,i}, \;\;\; i=1,\dots,m,
\label{eq2.3}
\ee
where $k_{\perp,i} n = k_{\perp,i} \bar n = 0$, $n^2 = {\bar n}^2 = 0$ and $n \bar n = 2$.  The two vectors $n$ and $\bar n$ can be thought of as the
(normalized) four-momenta of the two partons $a$ and $\bar{a}$ that produce the color-singlet final state
at leading order. In this parametrization
the phase-space element reads 
\be
\begin{split} 
&  [{\rm d} k_i] = \frac{{\Omega}^{(d-2)}
}{4 (2 \pi)^{d-1} } \;  {\rm d} \alpha_i \; {\rm d} \beta_i \; (\alpha_i \beta_i )^{-\ep} \;
\frac{ {\rm d} {\Omega}_{i,\perp}^{(d-2)}}{{\Omega}^{(d-2)}} \,, ~~~ \alpha_i\,,\beta_i \in [0,\infty] \,.
\end{split} 
\label{eq2.8a}
\ee



Using the Sudakov decomposition in Eq.~(\ref{eq2.3}), we can write 
\be
{\cal T} = \sum \limits_{i=1}^{m} {\rm min} \left \{ \alpha_i,\beta_i \right \}.
\ee
To make the choice between $\alpha_i$ and $\beta_i$ obvious in the above equation,  we can  partition the phase space by writing 
\be
1 = \theta(\alpha_i - \beta_i) + \theta(\beta_i - \alpha_i),
\label{eq2.5}
\ee
for each of the $m$ gluons.
It is clear  that  the first term will contribute $\beta_i$  and the second one $\alpha_i$ to
the jettiness variable ${\cal T}$.

Inserting the partition Eq.~(\ref{eq2.5}) into the integral
in Eq.~(\ref{eq2.1}) for each of the $m$ gluons, we obtain $2^m$ different terms.
However, using the symmetry between  $m$ gluons and the fact that the result is invariant
under the simultaneous replacement of all $\alpha_i$'s with $\beta_i$'s and vice versa,
we come to the conclusion that, for $m \le 3$,   only two independent cases need  to be considered.
They  are 1)
all $m$ gluons are emitted into the same hemisphere and  2)
all but one gluons are emitted into the
same hemisphere.

To derive the representation of  the soft function that we will use  in the remainder of  this paper, we 
re-scale  momenta $k_i \to k_i \tau$ and use  the fact that the eikonal function is a homogeneous, fully-symmetric 
function of gluon four-momenta. It follows 
\be
{\rm Eik}_{mg}(\tau k_1, \dots , \tau k_m,n,\bar n) = \tau^{-2m} {\rm Eik}_{mg}(k_1, \dots, k_m,n,\bar n).
\ee
Using re-scaled momenta, we can  write gluonic real-emission contributions to the soft
functions at NNLO and N3LO as follows
\begin{align}
\label{eqn:S2g_def}
S^{(2g)}(\tau) ={} & \tau^{-1-4\ep} \left[ S_{nn} + S_{n\bar n} \right] , \\
\label{eqn:S3g_def}
S^{(3g)}(\tau) ={} & \tau^{-1-6\ep} \left[ \frac1{3} S_{nnn} + S_{nn\bar n} \right] \,.
\end{align}
In Eqs.~(\ref{eqn:S2g_def},\ref{eqn:S3g_def}), we defined
\begin{align}
\begin{split} 
  & S_{nn} =
    \int \mathrm{d} \Phi^{nn}_{\theta\theta}  {\rm Eik}_{2g}(\{k_i\},n,\bar n), ~~~ S_{n\bar n} =
     \int  \mathrm{d} \Phi^{n\bar{n}}_{\theta\theta}  \; {\rm Eik}_{2g}(\{k_i\},n,\bar n),
\end{split} 
\label{eqn:n2lo_hemi_def}
\end{align}
and
\begin{align}
\begin{split} 
  S_{nnn} =
  \int \mathrm{d} \Phi^{nnn}_{\theta\theta\theta}   \; {\rm Eik}_{3g}(\{k_i\},n,\bar n), ~~~
  S_{nn\bar n} = \int \mathrm{d} \Phi^{nn\bar{n}}_{\theta\theta\theta}  \; {\rm Eik}_{3g}(\{k_i\},n,\bar n),
\end{split} 
\label{eqn:n3lo_hemi_def}
\end{align}
where 
\begin{align}
\label{eqn:ps_withf_general}
\mathrm{d} \Phi^{h_1,\dots,h_m}_{f_1,\dots,f_m} = (N_\ep)^{-m} \left( \prod \limits_{j=1}^{m} [{\rm d} k_j] f_j(\Delta_{j,h_j}) \right) \;  \delta (1 - \sum_{j=1}^{m} \kappa_{j,h_j})\,,
\end{align}
with
\begin{align}
\Delta_{j,h_j} ={} &
\begin{cases} 
\alpha_j-\beta_j \,, & h_j = n \,, \\
\beta_j-\alpha_j \,, & h_j = \bar{n} \,,
\end{cases} 
\;\;\;\;\;\; {\rm and}\;\;\;\;\;\; \kappa_{j,h_j} ={} 
\begin{cases} 
\beta_j \,, & h_j = n \,, \\
\alpha_j \,, & h_j = \bar{n} \,.
\end{cases}
\end{align}

To compute the zero-jettiness soft function  through N3LO in perturbative QCD the following phase spaces are needed
\begin{align}
 \mathrm{d} \Phi^{nn}_{\theta\theta} ={} & N_\ep^{-2} \left( \prod \limits_{j=1}^{2} [{\rm d} k_j] \theta(\alpha_j - \beta_j) \right) \;  \delta (1 - \beta_{12}) \,,\\
 \mathrm{d} \Phi^{n\bar{n}}_{\theta\theta} ={} & N_\ep^{-2} [{\rm d} k_1] \theta(\alpha_1 - \beta_1) \; [{\rm d} k_2] \theta(\beta_2 - \alpha_2) \; \delta (1 - \beta_1-\alpha_2) \,, \\
\mathrm{d} \Phi^{nnn}_{\theta\theta\theta} = {} & N_\ep^{-3} \left( \prod \limits_{j=1}^{3} [{\rm d} k_j] \theta(\alpha_j - \beta_j) \right) \;  \delta (1 - \beta_{123}) \,, \\
 \mathrm{d} \Phi^{nn\bar{n}}_{\theta\theta\theta} = {} & N_\ep^{-3} \left( \prod \limits_{j=1}^{2}  [{\rm d} k_j] \theta(\alpha_j - \beta_j) \right) \; [{\rm d} k_3] \theta(\beta_3 - \alpha_3) \; \delta (1 - \beta_{12} - \alpha_3) \,.
\end{align}
We note that we have used a shorthand notation  $\beta_{123} = \beta_1 + \beta_2 + \beta_3$ and $\beta_{12} = \beta_1 + \beta_2$
 in the above formulas. 


 The eikonal functions ${\rm Eik}_{2g}$ and ${\rm Eik}_{3g}$, that appeared in Eqs.~(\ref{eqn:n2lo_hemi_def},\ref{eqn:n3lo_hemi_def}),
 read\footnote{We recall, that we have factored out powers of $g_{s,b}$ in Eq.~(\ref{eqn:pert_exp_softF}).}
\begin{align}
\label{eqn:eik2g_def}
& {\rm Eik}_{2g}(k_1,k_2,n,\bar{n}) ={} C_a^2 \times \left[ \omega^{(1)}_{n\bar{n}}(k_1) \, \omega^{(1)}_{n\bar{n}}(k_2) \right] + C_a C_A \times \omega^{(2)}_{n\bar{n}}(k_1,k_2) \,, \\
\label{eqn:eik3g_def}
& {\rm Eik}_{3g}(k_1,k_2,k_3,n,\bar{n}) ={}  C_a^3 \times \left[ \omega^{(1)}_{n\bar{n}}(k_1) \, \omega^{(1)}_{n\bar{n}}(k_2) \, \omega^{(1)}_{n\bar{n}}(k_3) \right ] \nonumber \\
&\;\;\;\;\;\;\;\;\;\;\;\;\;\;\; +  C_a^2 C_A \times \left[ \omega^{(1)}_{n\bar{n}}(k_1) \, \omega^{(2)}_{n\bar{n}}(k_2,k_3) + (k_1 \leftrightarrow k_2) + (k_1 \leftrightarrow k_3) \right ] \nonumber \\
& \;\;\;\;\;\;\;\;\;\;\;\;\;\;\; +  C_a C_A^2 \times \omega^{(3)}_{n\bar{n}}(k_1,k_2,k_3) \,,
\end{align}
where $C_a=C_F$ ($C_a=C_A$) if $a\bar{a}=q\bar{q}$ ($a\bar{a}=gg$). The two quantities 
$C_F=(N_c^2-1)/(2N_c)$ and $C_A=N_c$ are the Casimir operators  of the SU($N_c$) algebra.
Functions $\omega^{(k)}_{n\bar{n}}(\{k_i\})$ in Eqs.~(\ref{eqn:eik2g_def},\ref{eqn:eik3g_def}) have been derived in Refs.~\cite{Catani:1999ss,Catani:2019nqv} and we borrow them from that reference.
Furthermore, we note that only maximally non-abelian contributions (given by terms 
proportional to $C_A$ and $C_A^2$ in Eqs.~(\ref{eqn:eik2g_def},\ref{eqn:eik3g_def}))  involve momenta of all radiated gluons at the respective order in perturbation theory. All other terms factorize and can be obtained from lower-order results. For this reason we will only
focus on the genuine NNLO and N3LO contributions to the zero-jettiness soft function and employ the
replacement 
\begin{align}
\label{eqn:eik2g_def_mnab}
{\rm Eik}_{2g}(k_1,k_2,n,\bar{n}) \, \longrightarrow  \,  {}& C_a C_A \times \omega^{(2)}_{n\bar{n}}(k_1,k_2) \,, \\
\label{eqn:eik3g_def_mnab}
{\rm Eik}_{3g}(k_1,k_2,k_3,n,\bar{n}) \, \longrightarrow \, {} & C_a C_A^2 \times \omega^{(3)}_{n\bar{n}}(k_1,k_2,k_3) \,.
\end{align}

As we already mentioned,   computation of integrals shown in  Eqs.~(\ref{eqn:n2lo_hemi_def},\ref{eqn:n3lo_hemi_def})
is made complicated because they contain $\theta$-functions of gluon momenta.
A standard way to simplify computation of complex phase-space integrals is to use reverse unitarity~\cite{Anastasiou:2002yz}
to map such integrals onto cut loop integrals for which IBP identities can be derived in a straightforward manner. However, it is not entirely clear how to work with $\theta$-functions in this context. For example, the authors of Refs.~\cite{Monni:2011gb,Kelley:2011ng} computed the NNLO zero-jettiness soft function by direct phase-space integration without relying on IBP relations. 
Alternatively, as was pointed out by one of us in  Ref.~\cite{Baranowski:2020xlp},
it is possible to make  phase-space  integrals with Heaviside-functions 
amenable to IBP techniques by  rewriting them
through parametric integrals using the relation\footnote{See also Section 4.2.2 in Ref.~\cite{Angeles-Martinez:2018mqh}.}
\begin{align}
\label{eqn:theta_as_delta}
\theta (b-a) = \int_{0}^{1} \mathrm{d} z \, \delta(z \, b -a ) \, b \,,  ~~~ a,b >0 \,.
\end{align}
While this representation yields an integrand whose dependence on  $z$ 
can be computed using reverse unitarity, it also
introduces one additional parametric integral per $\theta$-function, which can become quite cumbersome.
For this reason, in this paper  we would like to investigate how to derive and use
IBP relations for phase-space integrals with $\theta$-functions \textit{directly}.









